The future is different: Large pre-trained language models fail in prediction tasks

Large pre-trained language models (LPLM) have shown spectacular success when fine-tuned on downstream supervised tasks. Yet, it is known that their performance can drastically drop when there is a distribution shift between the data used during training and that used at inference time. In this paper we focus on data distributions that naturally change over time and introduce four new REDDIT datasets, namely the WALLSTREETBETS, ASKSCIENCE, THE DONALD, and POLITICS sub-reddits. First, we empirically demonstrate that LPLM can display average performance drops of about 88% (in the best case!) when predicting the popularity of future posts from sub-reddits whose topic distribution changes with time. We then introduce a simple methodology that leverages neural variational dynamic topic models and attention mechanisms to infer temporal language model representations for regression tasks. Our models display performance drops of only about 40% in the worst cases (2% in the best ones) when predicting the popularity of future posts, while using only about 7% of the total number of parameters of LPLM and providing interpretable representations that offer insight into real-world events, like the GameStop short squeeze of 2021

==> topic_trends.tex <==
\subsection{Modelling topic trendiness}

As I understood it, one of the original ideas of the model was to capture the context in the evolving document collection which makes some documents trendier than others. 
%
One could imagine a second \textbf{global} latent variable that weights the trendiness of \textbf{global} topics as time evolves. 
%
These \textbf{global} topics being represented by the topic embeddings $\+\alpha_i$.

Let these new random variable be generated thus

\begin{equation}
    \+\xi_t = \mathcal{N}\left(\boldsymbol{\mu}^{\xi}_{\psi}(\+\xi_{t-1}), \+\delta \, \mathbf{I}\right)
\end{equation}
%
with posterior given by

\begin{equation}
q_{\varphi}(\+\xi_t|\+\xi_{t-1},\*W_{1:T}) =  \mathcal{N}(\+\mu^{\xi}_{\varphi}[\+\xi_{t-1}, \*h^{\xi}_t],\+\sigma^{\xi}_{\varphi}[\+\xi_{t-1}, \*h^{\xi}_t]),
\end{equation}
%
where, just as in Eq.~\eqref{eq:posterior_global_1} above, $\+\mu^{\xi}_{\varphi}, \+\sigma^{\xi}_{\varphi}$ are neural networks and
\begin{equation}
\*h^{\xi}_t = g^{\xi}_{\varphi}(\*W_t, \*h^{\xi}_{t-1}).
\label{eq:posterior_global_2}
\end{equation}

We can then define a dynamic set of trendy topics as 

\begin{equation}
    \+\alpha_{t, i} = \text{exp}\left[\frac{1}{\sqrt{E}}(\*M^{\alpha}_{Q} \cdot \+\xi_t) \cdot (\*M^{\alpha}_{K} \cdot \+\alpha_i)^T\right] \odot (\*M^{\alpha}_V \cdot \+\alpha_i),
\end{equation}

and the summary document representations as

\begin{equation}
    \*s_{d} = \sum_i^K \sum_j^N \left( \theta_{t, d}^{(i)} \odot \text{softmax}\left[ \frac{1}{\sqrt{E}} (\*M^{u}_{Q} \cdot \+\alpha_{t, i}) \cdot (\*M^{u}_{K} \cdot \*u_j)^T \right]\right) \cdot (\*M^{u}_V \cdot \*u_j) + \*u_j,
    \label{eq:trendy_topics}
\end{equation}


\section{Possible problems with the model:}

\begin{enumerate}
    \item \textbf{Encoding rating information}. Given that we are not following specific writers in time, there is no rating time series available, is it?
    %
    Furthermore, to try to define a global rating variable seems flawed, for the ratings are conditioned entirely on local documents, not on collections of them.
    %
    In contrast, topics exist in the space of aggregated documents, due to precisely the word exchangeability assumption and the counting co-occurrence feature underlying topic models. 
    %
    A similar assumption can't clearly hold for document ratings, and if it can, I myself can't really see it. 
    \item \textbf{Fitting unsupervised representations (as e.g. topics) for supervised (i.e. regression or classification) tasks can be suboptimal}. This is actually the main point of \cite{pmlr-v108-wang20c}. 
    %
    We don't need, of course, to believe them (although it kind of makes sense). We can simply try and solve our supervised task from the representation inferred via a Dynamic Topic Model (DTM) alone and compare against e.g. BERT. 
\end{enumerate}

\subsection{Dynamic topic model with attention over pretrained models}

An clear generalization of the model above consists of:

\begin{enumerate}[label=(\roman*)]
    \item replacing $s_{\psi}$ above with a pretrained language models (so that the $\*u_i$ are now contextual word representations),
    \item using the dynamic topic proportions to weight the topic summation.
\end{enumerate}

Indeed we can rewrite Eq.~\eqref{eq:attention_topic} as

\begin{equation}
    \*s_d = \sum_j^N\sum_i^K (\theta_{t,d}^i - \delta) \, \text{softmax}(\text{MLP}(\*u^{(d)}_j)^T \cdot \+\alpha_i) \, \*u^{(d)}_j,
    \label{eq:attention_topic}
\end{equation}
%
the only difference being the time index $t$ on the topic proportions, and that the $\*u^{(d)}_j$ are now contextual word representations from a large pretrained language model.
